Early Detection of Security-Relevant Bug Reports using Machine Learning: How Far Are We?

Bug reports are common artefacts in software development. They serve as the main channel for users to communicate to developers information about the issues that they encounter when using released versions of software programs. In the descriptions of issues, however, a user may, intentionally or not, expose a vulnerability. In a typical maintenance scenario, such security-relevant bug reports are prioritised by the development team when preparing corrective patches. Nevertheless, when security relevance is not immediately expressed (e.g., via a tag) or rapidly identified by triaging teams, the open security-relevant bug report can become a critical leak of sensitive information that attackers can leverage to perform zero-day attacks. To support practitioners in triaging bug reports, the research community has proposed a number of approaches for the detection of security-relevant bug reports. In recent years, approaches in this respect based on machine learning have been reported with promising performance. Our work focuses on such approaches, and revisits their building blocks to provide a comprehensive view on the current achievements. To that end, we built a large experimental dataset and performed extensive experiments with variations in feature sets and learning algorithms. Eventually, our study highlights different approach configurations that yield best performing classifiers.

==> discussion.tex <==
\section{Disscussion}
\subsection{Content choice}
 Figure~\ref{fig:f-measure bf} and Figure~\ref{fig:f-measure tf} show the F-measure results on our dataset with a highlight on with content used. For this experiment, we use TF and BF features, for each type of content (title content, description content and title+description content) we compute TF and BF features. As feature vectors size we took 100 for BF and TF. 

Figure~\ref{fig:f-measure bf} shows that for most algorithms, use a Binary Bag of Words on title with large size of feature vector could lead to null prediction, due to the high number of 0 in the binary vector. Only a few sets of algorithms are able to predict with an acceptable result in this case. Gaussian Naive Bayes (GNB), K-Nearest-Neighbors (KNN), Random Forest (RF), and SVC are the algorithms that predict best in this situation. We also notice that, with the BF feature set, it's better to us title+description content because it allows getting better results compare to using title content or description content.

Figure~\ref{fig:f-measure tf}  show that, for the most of supervised algorithms, TF feature set give better results if we use only description. However, some algorithms like Gradient Boosting(GB) and XGB have better F-score by using title+description content.

All these experiments show that results depend on the content used. Even if the data are not often available it is a good choice to use content that can allow achieving good prediction. Results show that title can be used for security bugs reports prediction but that doesn't guarantee good results every time and sometimes with some feature set like Binary Bag-of-word it could lead to prediction errors. Description and title+description content give better results than only title, in most cases title+description give better results with the three feature sets. However, some classifiers can get good predictions with the only description of bug reports if the using feature set is TF.  

\begin{figure}[ht]
\centering
\includegraphics[width=1.00\linewidth]{Early_detection_of_SBR/figs/graphs/compar/BF_F_Score.pdf}
\caption{F-measure BF}
\label{fig:f-measure bf}
\end{figure}

\begin{figure}[!h]
\centering
\includegraphics[width=1.00\linewidth]{Early_detection_of_SBR/figs/graphs/compar/TF_F_Score.pdf}
\caption{F-measure TF}
\label{fig:f-measure tf}
\end{figure}

\subsection{Feature choice}
Binary Bag-of-words (BF), Term Frequency (TF), Term Frequency-Inverse Document Frequency (TF-IDF) are common in text classification using machine learning. We have experimented with three approaches for feature extraction in security bugs reports detection for identifying the best feature set to use. Our results show that in most of the case, the TF-IDF feature-set perform the best F-score results with using all three types of contents.  

Term Frequency (TF) feature-set give also acceptable results on the identification of security bug reports. Results show that it is possible to achieve good results with TF features if we use description content or title+description content. 

Binary Bag-of-words (BF) feature set is simple to compute, however, the results show that using the BF feature gives the lowest performance compare to TF or TF-IDF. In some cases, if the number of words in bug reports is not enough, this can lead to null prediction metric-scores, due to the gradient disappearance.

Feature extraction is an important task in machine learning approaches, Our experiments show that choosing a good feature-set to extract have an important impact on prediction results. We notice that TF-IDF is better in terms of F-score prediction value.  


%\subsection{Type of machine learning approaches}
%\begin{figure}[!h]
%\centering
%\includegraphics[width=0.90\linewidth]{Early_detection_of_SBR/figs/loss.pdf}
%%\caption{Loss }
%\label{fig:loss}
%\end{figure}


%\begin{figure}[!h]
%\centering
%\includegraphics[width=0.90\linewidth]{Early_detection_of_SBR/figs/acc.pdf}
%\caption{Accuracy}
%\label{fig:accuracy}
%\end{figure}
Supervised learning: we have experimented with security bug reports classification with eleven supervised algorithms. It's revealing that supervised learning allows to achieve good prediction performances depending on the type of feature extracted, feature-vectors size, and content used. In the set of classifiers used, Trees (Extra Trees, Bagged Decision Trees 1 and 2), Gaussian Naive Bayes, AdaBoost 1 and 2 got the best classification performances. 

Deep learning in security bug reports detection is recent, to the best of our knowledge, there are no articles that have used deep learning to detect security-relevant bug reports. 
The results that we got using deep learning are also acceptable, however, in general terms, our experiments show that supervised learning approaches can achieve better results than CNN.


\begin{figure}[ht]
\begin{subfigure}{.5\textwidth}
  \centering
  % include first image
\includegraphics[width=1.00\linewidth, height=0.6\textwidth]{Early_detection_of_SBR/figs/graphs/tfidf/f1/Extra_Trees.pdf}
\caption{fig: ET results with variable feature-vector size}
\label{fp1}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  % include second image
\includegraphics[width=1.00\linewidth, height=0.6\textwidth]{Early_detection_of_SBR/figs/graphs/tfidf/f1/Gradient_Boosting.pdf}
  \caption{fig: GNB results with variable feature-vector size}
  \label{fp3}
\end{subfigure}
\caption{ vector size impact(1)}
\label{fig:results_feature_size1}
\end{figure}

\begin{figure}[ht]
\begin{subfigure}{.5\textwidth}
  \centering
  % include first image
\includegraphics[width=1.00\linewidth, height=0.6\textwidth]{Early_detection_of_SBR/figs/graphs/tfidf/f1/AdaBoost_1.pdf}
\caption{fig: ADA1 results with variable feature-vector size}
\label{fp1}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  % include second image
\includegraphics[width=1.00\linewidth, height=0.6\textwidth]{Early_detection_of_SBR/figs/graphs/tfidf/f1/AdaBoost_2.pdf}
  \caption{fig: ADA2 results with variable feature-vector size}
  \label{fp3}
\end{subfigure}
\caption{ vector size impact(2)}
\label{fig:results_feature_size2}
\end{figure}


\begin{figure}[ht]
\begin{subfigure}{.5\textwidth}
  \centering
  % include first image
\includegraphics[width=1.00\linewidth, height=0.6\textwidth]{Early_detection_of_SBR/figs/graphs/tfidf/f1/Bagged_Decision_Trees_1.pdf}
\caption{fig: BDT1 results with variable feature-vector size}
\label{fp1}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  % include second image
\includegraphics[width=1.00\linewidth, height=0.6\textwidth]{Early_detection_of_SBR/figs/graphs/tfidf/f1/Bagged_Decision_Trees_2.pdf}
  \caption{fig: BDT2 results with variable feature-vector size}
  \label{fp3}
\end{subfigure}
\caption{ vector size impact(3)}
\label{fig:results_feature_size3}
\end{figure}

==> machine.tex <==

\section{Machine learning approaches for security-relevant bugs reports detection}

In this section, we will highlight the building blocks behind existing approaches in security bug reports identification.  We will also investigate the limitations of these approaches to suggest better approaches for solving this problem.

Existing machine-learning approaches in the state of art differ mainly on their features extraction methods and their learning type used (supervised, semi-supervised and non-supervised).

 \subsubsection{Feature extraction}
In most cases, using machine learning for prediction required the availability of train and test data. Data collected might be directly readable by algorithms in their default nature. However the default data format is not always in a readable format for machine learning algorithms, the feature extraction phase is then required for these cases. Feature extraction then yields to get a representative and qualitative set of the default dataset that. This process produces data in a readable format for machine learning algorithms. We consider in this study many feature extraction approaches used in the state of art for extracting representative information in security bug reports detection. We can summarize the different approaches to feature extraction by:


%and we add also an approach that is commly used in text mining that is word embedding.


%Predicting on the data of a specific problem can have several requirements, when the data are directly readable by the model and represent the key entity of prediction (bug report for example), the extraction of features is not necessary, this is the case of learning approaches such as word embedding, natural language processing, etc. However, the data of the problem are not always in readable format for algorithms or is often too voluminous (e. g. +10k commits ) for put it directly as input to algortithm, a feature engineering step is require in these case. Although some authors say that the extraction of characteristics (feature engineering) has little influence on the prediction results~\cite{Goseva-Popstojanova2018}, it would be wise to consider the possibility of any influence on the model because it represents the link between the model and the raw data. 

%In the state of the art, several approaches to extract representative information in the text are used and these approaches have demonstrated their relevance through the prediction performance of the classifiers used. We can keep some popular approaches used for feature extraction:
\begin{itemize}
	\item ~\cite{Goseva-Popstojanova2018,Gegick2010,Behl2014,Das2019,Pereira2019} \textbf{Frequencies of words in the text}: Using frequencies of words to retrieve quantitative metrics TF/IDF, BF, DF, IDF, etc.
	\item ~\cite{Peters2019,Mostafa}\textbf{Keyword mining}: Mining a list of words related to a prediction class and using this list for prefiltering and/or for performing prediction results.
	%\item\textbf{word embedding}: Using relation between words to predict the nature of a bug report
\end{itemize}

\find{Results show that using the frequencies of words in the text provides a more complete representation of information and thus makes it possible to achieve better prediction results}



 \subsubsection{Machine learning approach}
  
  
Existing works on the identification of security bug reports by machine learning is divided into three classes.
 

\begin{itemize}


\item Supervised learning ~\cite{Goseva-Popstojanova2018,Gegick2010,Behl2014,Holcomb1997, Das2019} is the classic prediction problem in which there are two classes and labeled data from both classes (positive class as the targeted class and negative class) are available. The chosen machine learning algorithm is trained on one part of the data and predict on the other part. The main problem of this approach is that it is often difficult for a given problem to have labeled data from both classes. It could happen in some cases that only one class is labeled.
\item Semi-supervised learning ~\cite{Mostafa2019,mostafaautomatic} represents the case where only one class is labeled and correctly identified. Several algorithms perform semi-supervised learning for identifying security bug reports with good prediction results. However, This approach, although very interesting, got bad performances when the positive set is not enough representative for training.
\item The main difference between the previous approaches (supervised and semi-supervised) and the unsupervised approaches is the fact that in the unsupervised case the data are not labeled. The algorithm must then train and predict from unlabeled examples. An example of an unsupervised learning algorithm used in the state of art~\cite{Goseva-Popstojanova2018} is clustering, which is frequently used to group data with similar characteristics from a classification point of view. 
\end{itemize}


\subsubsection{validation}

There are several Validation approaches in security bug reports detection, existing works are divided between manual validation and automatic validation using oracle (k-fold-cross, random sample, etc.). Manual validation has the most confidence, it requires a security team to validate prediction results. This validation method is the most reliable in the sense that it provides strong proof.
However, automatic validation is the most widespread in the detection of security bugs with machine learning. In the state of art, common automatic validation techniques used are k-fol-cross-validation and random split validation.

%The typical scenario is the separation of data into two sets (training and test) and the test data will constitute the oracle once the training of the model is completed. This approach also allows discovering if the model can make good predictions. Some authors also combine the two approaches to fit size and confidence checking.The validation by the oracle is, however, the most widespread in the detection of security bugs with machine learning because of the huge size of data. The typical scenario is the separation of data into two sets (training and test) and the test data will constitute the oracle once the training of the model is completed. This approach also allows discovering if the model can make good predictions. Some authors also combine the two approaches to fit size and confidence checking.%

==> threats.tex <==
\section{Threats to Validity}
